DEHYDRATOR: Enhancing Provenance Graph Storage via Hierarchical Encoding and Sequence Generation

As the scope and impact of cyber threats have expanded, analysts utilize audit logs to hunt threats and investigate attacks. The provenance graphs constructed from kernel logs are increasingly considered as an ideal data source due to their powerful semantic expression and attack historic correlation ability. However, storing provenance graphs with traditional databases faces the challenge of high storage overhead, given the high frequency of kernel events and the persistence of attacks. To address this, we propose Dehydrator, an efficient provenance graph storage system. For the logs generated by auditing frameworks, Dehydrator uses field mapping encoding to filter field-level redundancy, hierarchical encoding to filter structure-level redundancy, and finally learns a deep neural network to support batch querying. We have conducted evaluations on seven datasets totaling over one billion log entries. Experimental results show that Dehydrator reduces the storage space by 84.55%. Dehydrator is 7.36 times more efficient than PostgreSQL, 7.16 times than Neo4j, and 16.17 times than Leonard (the work most closely related to Dehydrator, published at Usenix Security'23).

==> 3_overview.tex <==
\section{Overview}
\label{sec:overview}
\sn{} is an efficient storage system for provenance graphs. Its architecture, as illustrated in Figure~\ref{fig:overview}, can be divided into three parts: (\uppercase\expandafter{\romannumeral 1}) Pretreatment, (\uppercase\expandafter{\romannumeral 2}) Storage, and (\uppercase\expandafter{\romannumeral 3}) Query.
\par
\textbf{Pretreatment.} \sn{} utilizes mature audit frameworks~\cite{etw, linux_subsystem, dtrace_freebsd, redhat} to collect system-level logs and save them into the node table $NT$ and edge table $ET$. \sn{} logically views the unification of these two tables as a provenance graph $G(V,\ E)$, which is a common practice~\cite{cheng2023kairos, yang2023prographer}. Then \sn{} addresses three types of field-level redundancy through field mapping encoding. Finally, based on \textbf{Key Insight \uppercase\expandafter{\romannumeral 1}}, \sn{} stores the node table on a hard disk, while reserving the edge table for subsequent processing. After this stage, \sn{} obtains the encoded node table $NT_{en}$, edge table $ET_{en}$, and the mapping table $MT$. We give a more detailed description in Section~\ref{sec:sysdesign_preprocessing}.
\par
\textbf{Storage.} Based on \textbf{Key Insight \uppercase\expandafter{\romannumeral 2}}, \sn{} performs a hierarchical encoding for the encoded edge table $ET_{en}$, which can effectively improve the training speed and model performance. 
This is because DNNs are better at fitting high-dimensional dense data. 
% This is because \sn{} models the storage as a sequence generation task, and DNNs are better at fitting high-dimensional dense data. 
Similarly, the NLP (Natural Language Processing) domain uses word2vec encoding instead of one-hot encoding when vectorizing words. We explain the reasons for using hierarchical encoding before model training in more detail in Section~\ref{sec:storing_hierarchical_encoding}. Then, \sn{} selects a single-layer encoder-only transformer with specific capacity as the training model based on \textbf{Key Insight \uppercase\expandafter{\romannumeral 3}}. Finally, \sn{} constructs an Error Correction Table (ECT) to counter the character-level misprediction. After this stage, \sn{} obtains the merge mapping table $MTT$, the model $DNN$, and the error correction table $ECT$. There are more details in Section~\ref{sec:sysdesign_storing}.
\par
\textbf{Query.} Given a query point (i.e., an Identifier ID), \sn{} first encodes it by mapping table $MT$. Then, depending on the specific query task, \sn{} follows different query processes. For node queries, \sn{} searches in the node table $NT_{en}$ (stored in the database), decodes, and returns the result. For edge queries, \sn{} inputs them into the model $DNN$, corrects, decodes, and returns the result. For higher-level tasks (such as backtracking dependency graph queries), \sn{} achieves this through iterative incoming edge queries. We give a more detailed description in Section~\ref{sec:sysdesign_query}.

\begin{figure*}[h!t]
\centering
% \vspace{-0.5cm}
\scalebox{0.9}{
\includegraphics[width=\linewidth]{Figures/overview.pdf}
}
\caption{Overview of \sn{}}
\label{fig:overview}
\vspace{-0.5cm}
\end{figure*}

